Black-Litterman Portfolio Optimization with Noisy Intermediate-Scale Quantum Computers

In this work, we demonstrate a practical application of noisy intermediate-scale quantum (NISQ) algorithms to enhance subroutines in the Black-Litterman (BL) portfolio optimization model. As a proof of concept, we implement a 12-qubit example for selecting 6 assets out of a 12-asset pool. Our approach involves predicting investor views with quantum machine learning (QML) and addressing the subsequent optimization problem using the variational quantum eigensolver (VQE). The solutions obtained from VQE exhibit a high approximation ratio behavior, and consistently outperform several common portfolio models in backtesting over a long period of time. A unique aspect of our VQE scheme is that after the quantum circuit is optimized, only a minimal number of samplings is required to give a high approximation ratio result since the probability distribution should be concentrated on high-quality solutions. We further emphasize the importance of employing only a small number of final samplings in our scheme by comparing the cost with those obtained from an exhaustive search and random sampling. The power of quantum computing can be anticipated when dealing with a larger-size problem due to the linear growth of the required qubit resources with the problem size. This is in contrast to classical computing where the search space grows exponentially with the problem size and would quickly reach the limit of classical computers.

==> table/eta.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{table*}[t]

\begin{subtable}{\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ |c|c|c c c c c c c c c c c c c c c c| } 
   \hline
   & & IPG & HAS & MAR & VLO & GL & MDT & MMM & HPQ & ADSK & NUE & PLD & XEL & $\qquad$ & $\qquad$ & $\qquad$  & $\qquad$\\
   
  \hline
  \multirow{4}{4em}{QSVM}&$s_1s_2$ & 0.29 & 0.09 &  0.10 & 0.19 & 0.03 & 0.07 & 0.23 & 0.28 & 0.21 & 0.11 & 0.39 & 0.07 &&&&\\ 
  &$Y_1$ & 1  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &&&&\\
  &$Y_2$ & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 &&&&\\
  &$\eta_k$ & 0.57 & 0.18 & 0.20 & 0.38 & 0.06 & 0.14 & 0.46 & 0.55 & 0.41 & 0.22 & 0.79 & 0.14 &&&&\\
  \hline
  \multirow{4}{4em}{QNN}&$s_1s_2$ & 0.29 & 0.09 &  0.10 & 0.19 & 0.03 & 0.07 & 0.23 & 0.28 & 0.21 & 0.11 & 0.39 & 0.07 &&&&\\ 
  &$Y_1$ & 1  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &&&&\\
  &$Y_2$ & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 &&&&\\
  &$\eta_k$ & 0.57 & 0.18 & 0.20 & 0.38 & 0.06 & 0.14 & 0.46 & 0.55 & 0.41 & 0.22 & 0.79 & 0.14 &&&&\\
  \hline
  \multirow{4}{4em}{SVM}&$s_1s_2$ & 0.29 & 0.09 &  0.10 & 0.19 & 0.03 & 0.07 & 0.23 & 0.28 & 0.21 & 0.11 & 0.39 & 0.07 &&&&\\ 
  &$Y_1$ & 1  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &&&&\\
  &$Y_2$ & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 &&&&\\
  &$\eta_k$ & 0.57 & 0.18 & 0.20 & 0.38 & 0.06 & 0.14 & 0.46 & 0.55 & 0.41 & 0.22 & 0.79 & 0.14 &&&&\\
  \hline
  \multirow{4}{4em}{NN}&$s_1s_2$ & 0.29 & 0.09 &  0.10 & 0.19 & 0.03 & 0.07 & 0.23 & 0.28 & 0.21 & 0.11 & 0.39 & 0.07 &&&&\\ 
  &$Y_1$ & 1  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &&&&\\
  &$Y_2$ & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 &&&&\\
  &$\eta_k$ & 0.57 & 0.18 & 0.20 & 0.38 & 0.06 & 0.14 & 0.46 & 0.55 & 0.41 & 0.22 & 0.79 & 0.14 &&&&\\
  \hline
\end{tabular}
}
\caption{Case 1.}
\end{subtable}

%\hfill

\begin{subtable}{\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ |c|c|c c c c c c c c c c c c c c c c| } 
   \hline
   & & SPYG & SPYV & VO & VB & QQQ & VEA & VWO & AGG & EMB & JNK & VNQ & RWX & MBB & MUB & TIP & GLD\\

  
  \hline
  \multirow{4}{4em}{QSVM}&$s_1s_2$ & 0.90 & 1.00 &  0.85 & 0.83 & 0.92 & 0.95 & 0.88 & 0.97 & 0.80 & 0.93 & 0.93 & 0.95 & 0.97 & 0.83 & 0.85 &.0.72\\ 
  &$Y_1$ & 1& -1& 1& -1& -1& -1& -1& -1& 1& 1& -1& -1& -1& 1& 1& 1 \\
  &$Y_2$ & 2& 2& 2& 2& 2& 2& 2& 1& 1& 2& 2& 2& 1& 1& 2& 1 \\
  &$\eta_k$ & 1.80 & -2.00 &  1.70 & -1.65 & -1.85& -1.90 & -1.76& -0.97&  0.80 & 1.86& -1.85& -1.90 & -0.97&  0.83&  1.69&  0.72\\
  \hline
  \multirow{4}{4em}{QNN}&$s_1s_2$ & 0.29 & 0.09 &  0.10 & 0.19 & 0.03 & 0.07 & 0.23 & 0.28 & 0.21 & 0.11 & 0.39 & 0.07 &&&&\\ 
  &$Y_1$ & 1  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1&&&& \\
  &$Y_2$ & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 &&&&\\
  &$\eta_k$ & 0.57 & 0.18 & 0.20 & 0.38 & 0.06 & 0.14 & 0.46 & 0.55 & 0.41 & 0.22 & 0.79 & 0.14 &&&&\\
  \hline
  \multirow{4}{4em}{SVM}&$s_1s_2$ & 0.29 & 0.09 &  0.10 & 0.19 & 0.03 & 0.07 & 0.23 & 0.28 & 0.21 & 0.11 & 0.39 & 0.07&&&& \\ 
  &$Y_1$ & 1  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &&&&\\
  &$Y_2$ & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2&&&& \\
  &$\eta_k$ & 0.57 & 0.18 & 0.20 & 0.38 & 0.06 & 0.14 & 0.46 & 0.55 & 0.41 & 0.22 & 0.79 & 0.14 &&&&\\
  \hline
  \multirow{4}{4em}{NN}&$s_1s_2$ & 0.29 & 0.09 &  0.10 & 0.19 & 0.03 & 0.07 & 0.23 & 0.28 & 0.21 & 0.11 & 0.39 & 0.07 &&&&\\ 
  &$Y_1$ & 1  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &&&&\\
  &$Y_2$ & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 &&&&\\
  &$\eta_k$ & 0.57 & 0.18 & 0.20 & 0.38 & 0.06 & 0.14 & 0.46 & 0.55 & 0.41 & 0.22 & 0.79 & 0.14 &&&&\\
  \hline
\end{tabular}
}
\caption{Case 2.}
\end{subtable}

\caption{}
\label{table:eta}
\end{table*}

==> table/opt.tex <==
\begin{table*}[h!]

\begin{subtable}{\textwidth}
\centering
\begin{tabular}{ |c|c|c| }
\hline
Time segment & VQE AR & QAOA AR\\
\hline
1 & 0.979 & 0.721 \\
\hline
2 & 1.0 & 0.715 \\
\hline
3 & 0.914 & 0.612 \\
\hline
4 & 0.911 & 0.83 \\
\hline
5 & 0.992 & 0.892 \\
\hline
6 & 0.965 & 0.919 \\
\hline
7 & 0.97 & 0.871 \\
\hline
8 & 0.983 & 0.512 \\
\hline
9 & 1.0 & 0.923 \\
\hline
\end{tabular}
\caption{Case 1 (individual stocks) optimization results for VQE, QAOA and exhaustive search.}
\label{table:opt1}
\end{subtable}

\begin{subtable}{\textwidth}
\centering
\begin{tabular}{ |c|c|c|c|c|c|c|c|c| }
\hline
     Time segment     &  Train & Test & VQE & AR & QAOA & AR & Exact \\
\hline
   1 & 2007-12-31 $\sim$ 2012-12-17&  2012-12-24 $\sim$ 2013-12-16 & 1011101000110001 &0.97 &  &  &1111100011100000\\
\hline
   2 & 2008-12-29 $\sim$ 2013-12-16&  2013-12-23 $\sim$ 2014-12-25 & 0101011010010011 &1.0 &  &  &0001011011110001\\
\hline
   3 & 2009-12-28 $\sim$ 2014-12-15&  2014-12-22 $\sim$ 2015-12-14 & 0111001011100100 &0.96 &  &  &0000001011110111\\ 
\hline
   4 & 2010-12-27 $\sim$ 2015-12-14&  2015-12-21 $\sim$ 2016-12-12 & 0111000011100110 &0.96 &  &  & 0110001011110100\\
\hline
   5 & 2011-12-26 $\sim$ 2016-12-12&  2016-12-19 $\sim$ 2017-12-11 & 1011100010101100 &0.96 &  &  &1111110000110000\\
\hline   
   6 & 2012-12-24 $\sim$ 2017-12-11&  2017-12-18 $\sim$ 2018-12-10 & 1011100011110000 &0.93 &  &  & 1111111000100000\\
\hline   
   7 & 2013-12-23 $\sim$ 2018-12-10&  2018-12-17 $\sim$ 2019-12-09 & 1010111000110001 &0.97 &  &  & 1011101010100010\\
\hline   
   8 & 2014-12-22 $\sim$ 2019-12-09&  2019-12-16 $\sim$ 2020-12-07 & 1010101000110011 &0.92 &  &  & 1000100110110011\\
\hline   
   9 & 2015-12-21 $\sim$ 2020-12-07&  2020-12-14 $\sim$ 2021-12-06 & 1010101010110001 &0.94 &  &  & 1000101011010101\\
\hline
\end{tabular}
\caption{Case 2 (global assets) optimization results for VQE, QAOA and exhaustive search.}
\label{table:opt2}
\end{subtable}

\caption{Optimization solutions.}
\end{table*}

==> table/qml_scores.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{table*}[t]
\begin{subtable}{\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ |c|c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| } 
    \hline
    & \multicolumn{2}{c|}{IPG} & \multicolumn{2}{c|}{HAS}  & \multicolumn{2}{c|}{MAR} & \multicolumn{2}{c|}{VLO} & \multicolumn{2}{c|}{GL} & \multicolumn{2}{c|}{MDT} & \multicolumn{2}{c|}{MMM} & \multicolumn{2}{c|}{HPQ} & \multicolumn{2}{c|}{ADSK} & \multicolumn{2}{c|}{NUE} &  \multicolumn{2}{c|}{PLD} & \multicolumn{2}{c|}{XEL} & \multicolumn{2}{c|}{mean} \\
    %\multicolumn{2}{c}{$\qquad$} & \multicolumn{2}{c}{$\qquad$} & \multicolumn{2}{c}{$\qquad$} & \multicolumn{2}{c|}{$\qquad$} \\
    \hline
    & $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$ \\
   
    \hline
QSVM & 0.92 & 0.9 & 0.98 & 0.88 & 0.97 & 0.88 & 0.92 & 0.84 & 0.96 & 0.93 & 0.92 & 0.94 & 0.93 & 0.91 & 0.9 & 0.85 & 0.9 & 0.91 & 0.89 & 0.95 & 0.91 & 0.92 & 0.98 & 0.83 & 0.93  &  0.9 \\
\hline
QNN & 0.76 & 0.75 & 0.83 & 0.72 & 0.78 & 0.75 & 0.75 & 0.75 & 0.79 & 0.76 & 0.74 & 0.78 & 0.82 & 0.78 & 0.77 & 0.72 & 0.78 & 0.77 & 0.73 & 0.72 & 0.77 & 0.78 & 0.82 & 0.65 & 0.78  &  0.74 \\
\hline
SVM & 0.92 & 0.91 & 0.97 & 0.88 & 0.95 & 0.91 & 0.93 & 0.83 & 0.94 & 0.93 & 0.9 & 0.92 & 0.92 & 0.9 & 0.93 & 0.81 & 0.9 & 0.9 & 0.85 & 0.92 & 0.93 & 0.88 & 0.98 & 0.83 & 0.93  &  0.89 \\
\hline
NN & 0.86 & 0.87 & 0.93 & 0.76 & 0.95 & 0.82 & 0.86 & 0.75 & 0.96 & 0.86 & 0.86 & 0.87 & 0.93 & 0.86 & 0.91 & 0.74 & 0.86 & 0.86 & 0.85 & 0.93 & 0.91 & 0.83 & 0.98 & 0.71 & 0.91  &  0.82 \\
\hline
  
\end{tabular}}
\caption{Testing accuracy of 4 ML models for each assets in Case 1. Each score is the average of all 9 time segments.}
\end{subtable}

%\hfill

\begin{subtable}{\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ |c|c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| c c| } 
   \hline
    & \multicolumn{2}{c|}{SPYG} & \multicolumn{2}{c|}{SPYV}  & \multicolumn{2}{c|}{VO} & \multicolumn{2}{c|}{VB} & \multicolumn{2}{c|}{QQQ} & \multicolumn{2}{c|}{VEA} & \multicolumn{2}{c|}{VWO} & \multicolumn{2}{c|}{AGG} & \multicolumn{2}{c|}{EMB} & \multicolumn{2}{c|}{JNK} &  \multicolumn{2}{c|}{VNQ} & \multicolumn{2}{c|}{RWX} & \multicolumn{2}{c|}{MBB} & \multicolumn{2}{c|}{MUB} & \multicolumn{2}{c|}{TIP} & \multicolumn{2}{c|}{GLD} &\multicolumn{2}{c|}{mean} \\
    \hline
    & $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$ & $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$& $Y_1$ & $Y_2$\\
   
    \hline
QSVM & 0.97 & 0.87 & 0.93 & 0.92 & 0.93 & 0.88 & 0.91 & 0.91 & 0.96 & 0.86 & 0.93 & 0.92 & 0.9 & 0.87 & 0.96 & 0.93 & 0.92 & 0.84 & 0.96 & 0.92 & 0.92 & 0.92 & 0.91 & 0.92 & 0.96 & 0.9 & 0.95 & 0.9 & 0.93 & 0.93 & 0.89 & 0.91 & 0.93  &  0.9 \\
\hline
QNN & 0.85 & 0.79 & 0.72 & 0.78 & 0.79 & 0.8 & 0.8 & 0.72 & 0.86 & 0.71 & 0.71 & 0.75 & 0.72 & 0.75 & 0.83 & 0.74 & 0.77 & 0.73 & 0.71 & 0.8 & 0.75 & 0.74 & 0.75 & 0.75 & 0.8 & 0.75 & 0.78 & 0.74 & 0.73 & 0.76 & 0.75 & 0.71 & 0.77  &  0.75 \\
\hline
SVM & 0.96 & 0.9 & 0.92 & 0.91 & 0.9 & 0.87 & 0.91 & 0.88 & 0.97 & 0.86 & 0.92 & 0.89 & 0.89 & 0.9 & 0.96 & 0.91 & 0.94 & 0.86 & 0.96 & 0.91 & 0.91 & 0.9 & 0.9 & 0.92 & 0.93 & 0.91 & 0.94 & 0.91 & 0.91 & 0.92 & 0.9 & 0.9 & 0.93  &  0.9 \\
\hline
NN & 0.96 & 0.78 & 0.89 & 0.84 & 0.91 & 0.8 & 0.89 & 0.83 & 0.96 & 0.78 & 0.89 & 0.84 & 0.85 & 0.89 & 0.9 & 0.88 & 0.9 & 0.79 & 0.95 & 0.81 & 0.92 & 0.87 & 0.86 & 0.85 & 0.88 & 0.89 & 0.91 & 0.84 & 0.9 & 0.9 & 0.87 & 0.87 & 0.9  &  0.84 \\
\hline
\end{tabular}}
\caption{Testing accuracy of 4 ML models for each assets in Case 2. Each score is the average of all 9 time segments.}
\end{subtable}

\caption{}
\label{table:qml_scores}
\end{table*}

==> table/time.tex <==
\begin{table}
\begin{center}
\begin{tabular}{ |c|c|c| }
\hline
     Time segment  &  Train & Test  \\
\hline
   1 & 2007-12-31 $\sim$ 2012-12-17&  2012-12-24 $\sim$ 2013-12-16 \\
\hline
   2 & 2008-12-29 $\sim$ 2013-12-16&  2013-12-23 $\sim$ 2014-12-25 \\
\hline
   3 & 2009-12-28 $\sim$ 2014-12-15&  2014-12-22 $\sim$ 2015-12-14 \\ 
\hline
   4 & 2010-12-27 $\sim$ 2015-12-14&  2015-12-21 $\sim$ 2016-12-12 0\\
\hline
   5 & 2011-12-26 $\sim$ 2016-12-12&  2016-12-19 $\sim$ 2017-12-11\\
\hline   
   6 & 2012-12-24 $\sim$ 2017-12-11&  2017-12-18 $\sim$ 2018-12-10 \\
\hline   
   7 & 2013-12-23 $\sim$ 2018-12-10&  2018-12-17 $\sim$ 2019-12-09 \\
\hline   
   8 & 2014-12-22 $\sim$ 2019-12-09&  2019-12-16 $\sim$ 2020-12-07 \\
\hline   
   9 & 2015-12-21 $\sim$ 2020-12-07&  2020-12-14 $\sim$ 2021-12-06 \\
\hline
\end{tabular}
\caption{Training and testing periods for walk-forward backtesting.}
\label{table:time}
\end{center}
\end{table}

==> table/vqe_riskadj_return.tex <==
\begin{table}
\begin{subtable}{0.49\textwidth}
\centering
 \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
         Time segment & INDEX & NAIVE & MPT & BL exact & BL VQE & BL QAOA\\
         \hline
0 & 0.445 & 0.378 & 0.368 & 0.439 & 0.437 & 0.347 \\
\hline
1 & 0.214 & 0.186 & 0.163 & 0.207 & 0.207 & 0.221 \\
\hline
2 & -0.069 & -0.015 & 0.037 & 0.052 & 0.065 & 0.023 \\
\hline
3 & 0.164 & 0.184 & 0.102 & 0.105 & 0.162 & 0.136 \\
\hline
4 & 0.251 & 0.238 & 0.232 & 0.241 & 0.237 & 0.305 \\
\hline
5 & -0.044 & -0.034 & -0.154 & -0.041 & 0.007 & -0.036 \\
\hline
6 & 0.17 & 0.223 & 0.3 & 0.207 & 0.18 & 0.144 \\
\hline
7 & -0.318 & -0.392 & -0.394 & -0.372 & -0.373 & -0.46 \\
\hline
8 & 0.147 & 0.227 & 0.273 & 0.166 & 0.166 & 0.092 \\
\hline
mean & 0.107 & 0.111 & 0.103 & 0.112 & 0.121 & 0.086 \\
\hline

    \end{tabular}
}
\caption{CER and SR of back test results of exact solution for case 1 (individual stocks).}
\label{tab:riskadj1}
\end{subtable}


\begin{subtable}{0.5\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
         \hline
         Time segment & \multicolumn{2}{c|}{BL} & \multicolumn{2}{c|}{MPT} & \multicolumn{2}{c|}{NAIVE} & \multicolumn{2}{c|}{INDEX}\\
         \hline
           & CER & SR & CER & SR & CER & SR & CER & SR\\
           \hline
1 & 0.186 & 1.936 & -0.018 & -0.392 & 0.077 & 0.927 & 0.077 & 0.927 \\
\hline
2 & 0.046 & 0.609 & 0.086 & 1.227 & 0.076 & 1.185 & 0.076 & 1.185 \\
\hline
3 & -0.07 & -0.808 & -0.021 & -0.175 & -0.052 & -0.533 & -0.052 & -0.533 \\
\hline
4 & 0.045 & 0.598 & 0.045 & 0.634 & 0.044 & 0.613 & 0.044 & 0.613 \\
\hline
5 & 0.171 & 3.2 & 0.141 & 2.967 & 0.131 & 3.241 & 0.131 & 3.241 \\
\hline
6 & -0.091 & -0.292 & -0.062 & -0.198 & -0.047 & -0.377 & -0.047 & -0.377 \\
\hline
7 & 0.2 & 2.76 & 0.185 & 3.46 & 0.178 & 3.188 & 0.178 & 3.188 \\
\hline
8 & -0.101 & 0.542 & 0.004 & 0.786 & -0.145 & 0.422 & -0.145 & 0.422 \\
\hline
9 & 0.071 & 1.049 & 0.068 & 1.115 & 0.094 & 1.368 & 0.094 & 1.368 \\
\hline
mean &  0.051 & 1.067 & 0.048 & 1.047 & 0.04 & 1.115 & 0.04 & 1.115 \\
         \hline
    \end{tabular}
}
\caption{CER and SR of back test results of exact solution for case 2 (global assets).}
\label{tab:riskadj2}
\end{subtable}


\caption{Risk-adjusted returns.}
\label{tab:riskadj}
\end{table}
